The Role of Teacher Calibration in Knowledge Distillation

Knowledge Distillation (KD) has emerged as an effective model compression technique in deep learning, enabling the transfer of knowledge from a large teacher model to a compact student model. While KD has demonstrated significant success, it is not yet fully understood which factors contribute to improving the student's performance. In this paper, we reveal a strong correlation between the teacher's calibration error and the student's accuracy. Therefore, we claim that the calibration of the teacher model is an important factor for effective KD. Furthermore, we demonstrate that the performance of KD can be improved by simply employing a calibration method that reduces the teacher's calibration error. Our algorithm is versatile, demonstrating effectiveness across various tasks from classification to detection. Moreover, it can be easily integrated with existing state-of-the-art methods, consistently achieving superior performance.

==> Tables/result_base_temperature_scaling.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{KD results with temperature scaled teachers.} The table shows the teacher model's accuracy and the student model's accuracy under standard KD and temperature-scaled KD on CIFAR-100 dataset. ResNet56 is used for the student model which has an original accuracy of 73.73\%.  }
\label{tab:comparison}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
Teacher architecture & vgg19 & vgg13 & vgg16 & resnet110 & wrn-28-2 & wrn-16-3 & wrn-40-2 & ResNet18 & wrn-16-4 \\
                        Teacher accuracy & 74.10  & 74.48 & 74.66 & 75.22     & 75.53    & 75.98    & 76.55    & 77.43    & 77.69    \\
\midrule
KD                       & 72.90  & 73.99 & 73.39 & 74.98 & 75.40 & 75.37 & 74.90 & 74.36 & 75.33 \\
KD + Ours       & \textbf{73.37} & \textbf{74.33} & \textbf{73.90} & \textbf{75.39} & \textbf{76.12} & \textbf{75.95} & \textbf{75.20} & \textbf{74.68} & \textbf{75.95} \\
$\Delta$          & \textcolor{red}{+0.47} & \textcolor{red}{+0.34} & \textcolor{red}{+0.51} & \textcolor{red}{+0.41} & \textcolor{red}{+0.72} & \textcolor{red}{+0.58} & \textcolor{red}{+0.30} & \textcolor{red}{+0.32} & \textcolor{red}{+0.62} \\

\bottomrule
\end{tabular}
}


\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
Teacher architecture & ResNet34 & GoogleNet & wrn-40-4 & wrn-28-4 & resnet32x4 & wrn-16-6 & wrn-16-8 & ResNet50 \\
                        Teacher accuracy & 78.41    & 78.46     & 78.51    & 78.56    & 78.70       & 78.79    & 79.37    & 79.71    \\
\midrule
KD                       & 74.53 & 74.81 & 75.00 & 74.27 & 74.95 & 75.55 & 75.16 & 75.13 \\
KD + Ours       & \textbf{74.80} & \textbf{75.60} & \textbf{75.12} & \textbf{74.53} & \textbf{75.23} & \textbf{75.62} & \textbf{75.23} & \textbf{75.48} \\
$\Delta$          & \textcolor{red}{+0.27} & \textcolor{red}{+0.79} & \textcolor{red}{+0.12} & \textcolor{red}{+0.26} & \textcolor{red}{+0.28} & \textcolor{red}{+0.07} & \textcolor{red}{+0.07} & \textcolor{red}{+0.35} \\

\bottomrule
\end{tabular}
}

\end{table*}

% \begin{table}[t]
% \centering
% \caption{\textbf{KD results with temperature scaled teachers.} The table shows the teacher model's accuracy and the student model's accuracy under standard KD and temperature-scaled KD. ResNet56 is used for the student model which has an original accuracy of 73.73\%.  }
% \label{tab:comparison}

% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccc}
% \toprule
% Teacher & Teacher accuracy & KD & KD + Ours \\
% \midrule
% vgg19 & 74.10 & 72.90 & \textbf{73.37} \\
% vgg13 & 74.48 & 73.99 & \textbf{74.33} \\
% vgg16 & 74.66 & 73.39 & \textbf{73.90} \\
% resnet110 & 75.22 & 74.98 & \textbf{75.39} \\
% wrn-28-2 & 75.53 & 75.40 & \textbf{76.12} \\
% wrn-16-3 & 75.98 & 75.37 & \textbf{75.95} \\
% wrn-40-2 & 76.55 & 74.90 & \textbf{75.20} \\
% ResNet18 & 77.43 & 74.36 & \textbf{74.68} \\
% wrn-16-4 & 77.69 & 75.33 & \textbf{75.95} \\
% ResNet34 & 78.41 & 74.53 & \textbf{74.80} \\
% GoogleNet & 78.46 & 74.81 & \textbf{75.60} \\
% wrn-40-4 & 78.51 & 75.00 & \textbf{75.12} \\
% wrn-28-4 & 78.56 & 74.27 & \textbf{74.53} \\
% resnet32x4 & 78.70 & 74.95 & \textbf{75.23} \\
% wrn-16-6 & 78.79 & 75.55 & \textbf{75.62} \\
% wrn-16-8 & 79.37 & 75.16 & \textbf{75.23} \\
% ResNet50 & 79.71 & 75.13 & \textbf{75.48} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> Tables/result_imagenet_resnet34.tex <==
\begin{table*}[ht]
    \centering
        \caption{\textbf{Top-1 and top-5 accuracy (\%) on the ImageNet validation set.} We set ResNet-34 as the teacher and ResNet-18 as the student network. $\dagger$ represents the result implemented by ours which is the average of three trials, and the standard deviation is expressed within parentheses.}
    \renewcommand{\arraystretch}{1.1}
    \resizebox{0.95\textwidth}{!}{%
        \begin{tabular}{@{}ccc cccc cccccc@{}}
            \toprule
            \multicolumn{3}{c}{Method} & \multicolumn{4}{c}{Features} & \multicolumn{5}{c}{Logits} \\
            \cmidrule(lr){1-3} \cmidrule(lr){4-7} \cmidrule(lr){8-13}
            & Teacher & Student & AT & OFD & CRD & RevieKD & KD & $\text{KD + Ours}^\dagger$ & TAKD & DKD & $\text{MLLD}^\dagger$ & $\text{MLLD + Ours}^\dagger$ \\
            \midrule
            top-1 & 73.31 & 69.75 & 70.69 & 70.81 & 71.17 & 71.61 & 70.66 & 71.60 (0.05) & 70.78 & 71.70  & 71.60 (0.06) & \textbf{71.90 (0.02)} \\
            top-5 & 91.42 & 89.07 & 90.01 & 89.98 & 90.13 & 90.51 & 89.88 & 90.24 (0.12) & 90.16 & 90.41 & 90.68 (0.09) & \textbf{90.72 (0.04)} \\
            \bottomrule
        \end{tabular}
    }

    \label{tab:imagenet_resnet34}
\vspace{-4mm}
\end{table*}


==> Tables/result_imagenet_resnet50.tex <==
\begin{table*}[ht]
    \centering
       \caption{\textbf{Top-1 and top-5 accuracy (\%) on the ImageNet validation set.} We set ResNet-50 as the teacher and MobileNet-V1 as the student. $\dagger$ represents the result implemented by ours which is the average of three trials, and the standard deviation is expressed within parentheses.}
    \renewcommand{\arraystretch}{1.1}
    \resizebox{0.95\textwidth}{!}{%
    \begin{tabular}{@{}ccc cccc cccccc@{}}
        \toprule
        \multicolumn{3}{c}{Method} & \multicolumn{4}{c}{Features} & \multicolumn{5}{c}{Logits} \\
        \cmidrule(lr){1-3} \cmidrule(lr){4-7} \cmidrule(lr){8-13}
        & Teacher & Student & AT & OFD & CRD & RevieKD & KD & $\text{KD + Ours}^\dagger$ & TAKD & DKD & $\text{MLLD}^\dagger$ & $\text{MLLD + Ours}^\dagger$ \\
        \midrule
        top-1 & 76.16 & 68.87 & 69.56 & 71.25 & 71.37 & 72.56 & 68.58 & 71.55 (0.06) & 70.82 & 72.05 & 73.05 (0.07) &\textbf{73.09 (0.04)} \\
        top-5 & 92.86 & 88.76 & 89.33 & 90.34 & 90.41 & 91.00 & 88.98 & 90.43 (0.09) & 73.01 & 91.05 & 91.34 (0.04) &\textbf{91.43 (0.05)} \\
        \bottomrule
    \end{tabular}%
    }
 
    \label{tab:imagenet_resnet50}
\end{table*}

==> Tables/tace_sacc.tex <==
\begin{table*}[ht]
\centering
\caption{\textbf{Properties of Teacher Models and Student Models used in this paper}: 
This table presents various metrics for teacher models and their corresponding student models' accuracy trained with the standard KD method on the CIFAR-100 dataset.}
\renewcommand{\arraystretch}{1.2}
\label{tab:tace_sacc}  % \label은 \caption 뒤에 위치해야 함

% \resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multicolumn{7}{c}{\textbf{Teacher Properties}} & \multicolumn{2}{c}{\textbf{Student KD Accuracy (\%)}} \\
\cmidrule(r){1-7} \cmidrule(l){8-9}
% \textbf{Model} & \textbf{Accuracy (\%)} & \textbf{ECE (\%)} & $\text{ECE}_{o} (\%)$ & $\text{ECE}_{u} (\%)$ & \textbf{ACE (\%)} & \textbf{Params} & \textbf{WRN-16-2} & \textbf{ShuffleNetV2} \\
\textbf{Model} & \textbf{Accuracy (\%)} & \textbf{ECE (\%)} & \textbf{ECE\(_{o}\) (\%)} & \textbf{ECE\(_{u}\) (\%)} & \textbf{ACE (\%)} & \textbf{Params} & \textbf{WRN-16-2} & \textbf{ShuffleNetV2} \\
\midrule
VGG19      & 74.10 & 16.4723 & 16.4723 & 0.0000 & 0.1336 & 20.1M & 74.42 & 74.17 \\
VGG13      & 74.48 & 8.4570  & 8.3338  & 0.1232 & 0.1048 & 9.5M  & 74.99 & 75.40  \\
VGG16      & 74.66 & 12.8963 & 12.8946 & 0.0017 & 0.1194 & 14.8M & 74.67 & 74.98 \\
ResNet110  & 75.22 & 13.0475 & 13.0475 & 0.0000 & 0.1007 & 1.7M  & 75.48 & 77.04 \\
WRN-28-2   & 75.53 & 7.1268  & 7.1268  & 0.0000 & 0.0924 & 1.5M  & 75.71 & 76.72 \\
WRN-16-3   & 75.98 & 8.7114  & 8.6809  & 0.0305 & 0.0899 & 1.6M  & 76.07 & 77.01 \\
WRN-40-2   & 76.55 & 11.2194 & 11.2003 & 0.0191 & 0.1000 & 2.3M  & 75.51 & 76.11 \\
ResNet18   & 77.43 & 6.9784  & 6.8159  & 0.1625 & 0.0938 & 11.2M & 75.75 & 76.48 \\
WRN-16-4   & 77.69 & 7.5518  & 7.5394  & 0.0124 & 0.0833 & 2.8M  & 76.25 & 76.80  \\
ResNet34   & 78.41 & 9.5015  & 9.4911  & 0.0104 & 0.0902 & 21.3M & 76.03 & 76.62 \\
GoogLeNet  & 78.46 & 6.7732  & 6.7621  & 0.0111 & 0.0762 & 6.4M  & 76.29 & 76.55 \\
WRN-40-4   & 78.51 & 10.3410 & 10.3410 & 0.0000 & 0.0914 & 9.0M  & 75.76 & 76.26 \\
WRN-28-4   & 78.56 & 8.2353  & 8.2353  & 0.0000 & 0.0905 & 5.9M  & 75.59 & 76.90  \\
ResNet32x4 & 78.70 & 9.3010  & 9.2661  & 0.0349 & 0.0840 & 7.4M  & 76.16 & 76.55 \\
WRN-16-6   & 78.79 & 6.3329  & 6.3271  & 0.0058 & 0.0836 & 6.2M  & 76.36 & 77.53 \\
WRN-16-8   & 79.37 & 5.6263  & 5.5865  & 0.0398 & 0.0794 & 11.0M & 76.34 & 76.99 \\
ResNet50   & 79.71 & 7.6640  & 7.6640  & 0.0000 & 0.0790 & 23.7M & 76.12 & 76.91 \\
\bottomrule
\end{tabular}
% }
\end{table*}


==> Tables/tace_sacc_part.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Comparison of Teacher Models which has similar accuracy.} Evaluation of the KD Accuracy of student models WRN-16-2 and ShuffleNetV2 with WRN-40-4, and GoogLeNet teacher on the CIFAR100 dataset. Bold values denote superior performance in each category.}
\label{tab:tace_sacc_part}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc cc}
\toprule
\multicolumn{3}{c}{\textbf{Teacher}} & \multicolumn{2}{c}{\textbf{Student KD Accuracy(\%)}} \\
\cmidrule(r){1-3} \cmidrule(l){4-5}
\textbf{Model} & \textbf{Accuracy $\uparrow$(\%)} & \textbf{ACE $\downarrow$(\%)} & WRN-16-2 & ShuffleNetV2 \\
\midrule
WRN-40-4   & \textbf{78.51} & 0.0914 & 75.76 & 76.26  \\
GoogLeNet  & 78.46 & \textbf{0.0762} & \textbf{76.29} & \textbf{76.55} \\

\bottomrule
\end{tabular}
}
\end{table}

